Unipotent Ideals for Spin and Exceptional Groups

In the monograph arXiv:2108.03453, we define the notion of a unipotent representation of a complex reductive group. The representations we define include, as a proper subset, all special unipotent representations in the sense of Barbasch-Vogan and form the (conjectural) building blocks of the unitary dual. In arXiv:2108.03453 we provide combinatorial formulas for the infinitesimal characters of all unipotent representations of linear classical groups. In this paper, we establish analogous formulas for spin and exceptional groups, thus completing the determination of the infinitesimal characters of all unipotent ideals. Using these formulas, we prove an old conjecture of Vogan: all unipotent ideals are maximal. For $G$ a real reductive Lie group (not necessarily complex), we introduce the notion of a unipotent representation attached to a rigid nilpotent orbit (in the complexified Lie algebra of $G$). Like their complex group counterparts, these representations form the (conjectural) building blocks of the unitary dual. Using the atlas software (and the work of Adams-Miller-van Leeuwen-Vogan) we show that if $G$ is a real form of a simple group of exceptional type, all such representations are unitary.

==> Old_tables.tex <==

\begin{table}[H]
    \begin{tabular}{|c|c|c|} \hline
        $\OO$ & $\OO_1$ & $\Sigma_1$ \\ \hline
        $G_2(a_1)$ & $\widetilde{A}_1$ & $A_1$  \\ \hline
    \end{tabular}
    \caption{Orbits with birationally rigid covers in type $G_2$}
\end{table}



\begin{table}[H]
    \begin{tabular}{|c|c|c|} \hline
        $\OO$ & $\OO_1$ & $\Sigma_1$ \\ \hline
        $F_4(a_3)$ & $C_3(a_1)$ & $A_1$ \\ \hline
        $B_2$ & $A_2+\widetilde{A}+1$ & $A_1$ \\ \hline
    \end{tabular}
    \caption{Orbits with birationally rigid covers in type $F_4$}
\end{table}

\begin{table}[H]
    \begin{tabular}{|c|c|c|c|c|} \hline
        $\OO$ & $\OO_1$ & $\Sigma_1$ & $\OO_2$ & $\Sigma_2$ \\ \hline
        $A_2$ & $3A_1$ & $A_1$ & - & - \\ \hline
        $D_4(a_1)$ & $A_3+A_1$ & $A_1$ & - & - \\ \hline
        $2A_2$ & $A_2+A_1$ & $A_2$ & - & - \\ \hline
        $A_5$ & $A_4+A_1$ & $A_2$ & - & -  \\ \hline
        $E_6(a_3)$ & $A_5$ & $A_1$ & $D_5(a_1)$ & $A_2$ \\ \hline
    \end{tabular}
    \caption{Orbits with birationally rigid covers in type $E_6$}
\end{table}


\begin{table}[H]
    \begin{tabular}{|c|c|c|c|c|c|c|} \hline
        $\OO$ & $\OO_1$ & $\Sigma_1$ & $\OO_2$ & $\Sigma_2$ & $\OO_3$ & $\Sigma_3$ \\ \hline
        $E_7(a_4)$ & $A_6$ & $A_1$ & $D_5+A_1$ & $A_1$ & $D_6(a_1)$ & $A_1$ \\ \hline
        
        $E_7(a_5)$ & $D_6(a_2)$ & $A_1$ & $E_6(a_3)$ & $A_1$ & - & - \\ \hline
        $D_4(a_1)+A_1$ & $D_4(a_1)$ & $[3A_1]^{++}$ & $A_3+2A_1$ & $A_1$ & - & - \\ \hline
        $A_5+A_1$ & $A_4+A_2$ & $A_1$ & - & - & - & - \\ \hline
        $A_3+A_2+A_1$ & $A_3+A_2$ & $A_1$ & - & - & - & - \\ \hline
        $D_4(a_1)$ & $(A_3+A_1)'$ & $A_1$ & - & - & - & - \\ \hline
        $A_3+2A_1$ & $(A_3+A_1)'$ & $A_1$ & - & - & - & - \\ \hline
        $(A_3+A_1)''$ & $2A_2$ & $A_1$ & $A_3$ & $A_1$ & - & - \\ \hline
        $A_2+3A_1$ & $A_2+2A_1$ & $A_1$ & - & - & - & - \\ \hline
        $A_2$ & $(3A_1)'$ & $A_1$ & - & - & - & - \\ \hline
    \end{tabular}
    \caption{Orbits with birationally rigid covers in type $E_7$}
\end{table}


\begin{table}[H]
    \begin{tabular}{|c|c|c|c|c|} \hline
        $\OO$ & $\OO_1$ & $\Sigma_1$ & $\OO_2$ & $\Sigma_2$ \\ \hline
        $E_8(b_6)$ & $E_6(a_1)+A_1$ & $A_2^+$ & $A_7$ & $A_1$  \\ \hline
        $A_2$ & $3A_1$ & $A_1$ & - & -  \\ \hline
        $2A_2$ & $A_2+3A_1$ & $A_1$ & - & -  \\ \hline
        $D_4(a_1)$ & $A_3+A_1$ & $A_1$ & - & -  \\ \hline
        $D_4(a_1)+A_2$ & $A_3+A_2+A_1$ & $A_1$ & - & -  \\ \hline
        $D_4+A_2$ & $D_5(a_1)+A_1$ & $A_1$ & $A_4+A_2+A_1$ & $A_1$  \\ \hline
        $E_6(a_3)+A_1$ & $A_5+A_1$ & $A_1$ & - & -  \\ \hline
        $D_6(a_2)$ & $D_5(a_1)+A_2$ & $A_1$ & - & -  \\ \hline
        $E_7(a_5)$ & $D_6(a_2)$ & $[2A_1]^{+}$ & - & -  \\ \hline
        $E_8(a_7)$ & $E_7(a_5)$ & $A_1$ & - & -  \\ \hline
    \end{tabular}
    \caption{Orbits with birationally rigid covers in type $E_8$}
\end{table}






==> notes.tex <==

In \cite{LMBM}, we de\cite{LMBM}, we fine, for each (finite, connected) $G$-equivariant covering $\widetilde{\OO}$ of a nilpotent co-adjoint orbit, a completely prime primitive ideal $I_0(\widetilde{\OO})$ in the enveloping algebra of $\fg$. We call $I_0(\widetilde{\OO})$ the \emph{unipotent ideal} attached to $\widetilde{\OO}$. A \emph{unipotent representation} attached to $\widetilde{\OO}$ is an irreducible Harish-Chandra bimodule for $U(\fg)$ which is annihilated (on both sides) by $I_0(\widetilde{\OO})$. We show in \cite{LMBM} that unipotent ideals and representations have many of the expected properties, including:

\begin{enumerate}
    \item All special unipotent ideals and representations (in the sense of \cite{BarbaschVogan1985}) are unipotent.
    \item The set of unipotent representations attached to $\widetilde{\OO}$ is in natural bijection with irreducible representations of a finite group, generalizing Lusztig's canonical quotient.
    \item Unipotent representations are, as representations of $K$, of the form conjectured by Vogan (see \cite[Conj 12.1]{Vogan1991}).
    \item For linear classical groups, unipotent ideals are maximal.
    \item For linear classical groups, unipotent representations are unitary.
\end{enumerate}

==> retired_criterion_rigid.tex <==

Finally, if $\mathbb{O}_K$ is one of the 6 exceptions listed in Proposition \ref{prop:mult1ideals}, there are several multiplicity-1 primitive ideals with associated variety $\overline{\mathbb{O}}_K$. Denote them by $I_0(\mathbb{O}_K),I_1,...,I_m \subset U(\mathfrak{k})$. In all six cases, Premet has computed at least two ideals, see \cite{Premet2013}, and all of his ideals are maximal. In four cases, he has proved that his list of ideals is exhaustive. In these four cases we can appeal to the following lemma to identify the unipotent ideal $I_0(\OO_K)$.

\begin{lemma}\label{lem:6exceptions}
Assume $I_0(\mathbb{O}_K)$ and $I_i$ ($1\leq i \leq m$) are maximal ideals in $U(\mathfrak{k})$. Then as $K$-representations
%
$$U(\mathfrak{k})/I_0(\mathbb{O}_K) \simeq_K \CC[\mathbb{O}_K] \qquad U(\mathfrak{k})/I_i \hookrightarrow_K \CC[\mathbb{O}_K] \quad 1 \leq i \leq m$$
%
and the embeddings $U(\mathfrak{k})/I_i \hookrightarrow_K \CC[\mathbb{O}_K]$ are strict.
\end{lemma}

\begin{proof}
Consider the W-algebra $\cW$ for $\mathbb{O}_K$ and the functors $\bullet_\dagger,\bullet^\dagger$ constructed in Section \ref{subsec:W}. By (iv) of \cref{lem:Adagger}, $I_0(\mathbb{O}_K)=J^\ddag$ for some $\pi_1(\OO_K)$-invariant ideal $J \subset \cW$ of codimension 1, and by Theorem \ref{thm:daggersurjective}, $I_0(\OO_K)_{\dagger} = J$. By (ii) and (iii) of Lemma \ref{lem:Adagger}, $\cA_0^{X_K} \xrightarrow{\sim} (\cW/J)^{\dagger} \xrightarrow{\sim} [(U(\mathfrak{k})/I_0(\OO_K))_{\dagger}]^{\dagger}$. Since $I_0(\OO_K)$ is maximal, Lemma \ref{lem:adjunctionmorphismiso}, applied to $U(\mathfrak{k})/I_0(\OO_K) \in \HC^K_{\overline{\OO}_K}(U(\mathfrak{k}))$, implies that the natural map $U(\mathfrak{k})/I_0(\OO_K) \to   ([U(\mathfrak{k})/I_0(\OO_K)]_{\dagger})^{\dagger}$ is an isomorphism. So  $U(\mathfrak{k})/I_0(\OO_K) \simeq \cA_0^{X_K}$ in $\HC^K_{\overline{\OO}_K}(U(\mathfrak{k}))$. Taking associated gradeds, we get an isomorphism of $K$-representations
%
$$\gr(U(\mathfrak{k})/I_0(\mathbb{O}_K)) \simeq_K \gr(\cA_0^{X_K}) \simeq_K \CC[\mathbb{O}_K].$$
%
It remains to exhibit strict embeddings $U(\mathfrak{k})/I_0(\OO_K) \hookrightarrow_K \CC[\OO_K]$ for $1 \leq i\leq m$. By Lemma \ref{lem:adjunctionmorphismiso},
there is a $K$-equivariant isomorphism $U(\mathfrak{k})/I_i\xrightarrow{\sim} [(U(\mathfrak{k})/I_i)_\dagger]^\dagger$. Note that  $(I_{i})_\dagger\subset \cW$ is a $\pi_1(\mathbb{O})$-invariant ideal of codimension 1. Thus by Lemma 
\ref{Lem:upper_dag_1dim}, there is an $K$-equivariant embedding $\gr [(U(\mathfrak{k})/I_i)_\dagger]^\dagger\hookrightarrow \C[\mathbb{O}_K]$. Suppose for contradiction that this embedding is an isomorphism. Then $[(U(\mathfrak{k})/I_i)_\dagger]^\dagger$ is a quantization of $\mathbb{C}[\mathbb{O}_K]$. Since $\OO_K$ is birationally rigid, $\cA_0^{X_K}$ is the unique filtered quantization of $\CC[\OO_K]$, see Corollary \ref{cor:criterionbirigid}. Hence $[(U(\mathfrak{k})/I_i)_\dagger]^\dagger \simeq \cA_0^{X_K}$, and therefore $I_i=I_0(\OO_K)$. This is a contradiction.
\end{proof}

In the cases in which Lemma \ref{lem:6exceptions} is applicable, {\fontfamily{cmtt}\selectfont
atlas} can be used to compare the $K$-types of the quotients $U(\mathfrak{k})/I_0(\OO_K)$ and $U(\mathfrak{k})/I_i$ and thus to identify $I_0(\OO_K)$.

\begin{example}
Let $K=G_2$ and let $\mathbb{O}_K=\widetilde{A}_1$ (i.e. the unique orbit of dimension 8). By \cite{Premet2013}, there are two multiplicity-free ideals attached to $\mathbb{O}_K$, namely the maximal ideals
%
$$I_1= I_{\mathrm{max}}(\frac{1}{2}\varpi_1+\frac{1}{2}\varpi_2) \qquad I_2=I_{\mathrm{max}}(\varpi_1 +\frac{1}{2}\varpi_2)$$
%
An {\fontfamily{cmtt}\selectfont atlas} computation shows that the irreducible 7-dimensional $K$-representation appears in $U(\mathfrak{k})/I_1$ (with multiplicity 1), but not in $U(\mathfrak{k})/I_2$. Thus, $I_1 = I_0(\mathbb{O}_K)$ by Lemma \ref{lem:6exceptions}. It is worth noting that $U(\mathfrak{k})/I_1$ is unitary, while $U(\mathfrak{k})/I_2$ is not (this follows, for example, from Duflo's classification of the unitary representations of complex groups of rank 2, see \cite{Duflo1979}).
\end{example}



